Locally Optimal Estimation and Control of Cable Driven Parallel Robots using Time Varying Linear Quadratic Gaussian Control

We present a locally optimal tracking controller for Cable Driven Parallel Robot (CDPR) control based on a time-varying Linear Quadratic Gaussian (TV-LQG) controller. In contrast to many methods which use fixed feedback gains, our time-varying controller computes the optimal gains depending on the location in the workspace and the future trajectory. Meanwhile, we rely heavily on offline computation to reduce the burden of online implementation and feasibility checking. Following the growing popularity of probabilistic graphical models for optimal control, we use factor graphs as a tool to formulate our controller for their efficiency, intuitiveness, and modularity. The topology of a factor graph encodes the relevant structural properties of equations in a way that facilitates insight and efficient computation using sparse linear algebra solvers. We first use factor graph optimization to compute a nominal trajectory, then linearize the graph and apply variable elimination to compute the locally optimal, time varying linear feedback gains. Next, we leverage the factor graph formulation to compute the locally optimal, time-varying Kalman Filter gains, and finally combine the locally optimal linear control and estimation laws to form a TV-LQG controller. We compare the tracking accuracy of our TV-LQG controller to a state-of-the-art dual-space feed-forward controller on a 2.9m x 2.3m, 4-cable planar robot and demonstrate improved tracking accuracies of 0.8{\deg} and 11.6mm root mean square error in rotation and translation respectively.

==> 2-0_preliminary.tex <==
We frame our approach around factor graphs because we believe them to be useful abstractions to describe trajectory optimization and controls topics.  Probabilistic graphical models, including factor graphs, have seen great success in state estimation and perception \cite{} and are becoming increasingly popular as tools for optimal control \cite{}.

A factor graph is, in rough terms, a way to graphically describe an optimization problem that visually reveals information about the sparsity of a problem.  More formally, a factor graph is a bipartite graph with variables and factors, where a variable represents an unknown to solve for and a factor represents a joint probability distribution over the variables it is connected to.  In the context of factor graphs for optimal control, we can alternatively interpret factors as cost objectives or constraint equations containing the connected variables.  Figure \ref{fig:standard_lqr} gives an example of the standard LQR problem described using a factor graph.  It is important to point out that, because factor graphs are \emph{probabilistic} graphical models, dynamics constraints may be interpreted as ``0-covariance'' joint distributions which require slightly modified algorithms to solve, but are nonetheless already studied.

Factor graphs are useful not only as visual aids, but also for the efficient algorithms developed to ``solve'' them, where we use the term ``solve'' to mean solving the optimization problem they describe: either computing the maximum a posteriori (MAP) estimate or constrained optimization minimization.

\begin{figure}
  \centering
  \includegraphics[page=1, trim=0 4.76in 7.28in+3pt 0, clip, width=\linewidth]{figs/figs.pdf}
  \caption{Prototypical example of a factor graph describing the LQR problem for 4 timesteps, where $x_k$ represent state variables, $u_k$ represent control variables, black squares represent dynamics constraint factors, and black circles represent optimal control objectives.}
  \label{fig:standard_lqr}
\end{figure}


==> 2-x_linearize.tex <==
Upon finding the solution, denoted $\xff, \uff$, we linearize the factor graph around $\xff, \uff$ and \emph{eliminate} the variables which are neither state nor control: cable length, cable velocity, cable acceleration, tension, wrench, and twist acceleration.
The first step creates a linear (``Gaussian'') factor graph and is equivalent to the 
and the second step solves for the variables 
which has the same structure as in Fig. \ref{fig:standard_lqr}.  The linearized graph is shown in Fig. \ref{fig:linearized_graph}.

\begin{figure}
    \centering
    \resizebox*{\linewidth}{!}{\input{figs/lqr_graph.tikz}}
    \caption{Linearized graph}
    \label{fig:linearized_graph}
\end{figure}

\todo{gerry}{Explain eliminating intermediate variables}

The linearization process is abstracted away and handled by GTSAM, but mathematically it can be described as applying a first-order Taylor expansion to linearize the dynamics around $\xff, \uff$:
\begin{align}
    x_{k+1} &\approx f_k(\xff, \uff) + \frac{\partial f_k}{\partial x}\left(x_k-\xff_k\right) + \frac{\partial f_k}{\partial u}\left(u_k-\uff_k\right) \\
        &= \xff_{k+1} + A(x_k-\xff_k) + B(u_k-\uff_k)
\end{align}

where we define $A_k \coloneqq \left.\frac{\partial f_k}{\partial x}\right\rvert_{(\xff, \uff)}$ and $B_k \coloneqq \left.\frac{\partial f_k}{\partial u}\right\rvert_{(\xff, \uff)}$.

Further defining $\deltax_k \coloneqq x_k-\xff_k$ and $\deltau_k \coloneqq u_k-\uff_k$, then 
\begin{align}
    \deltax_{k+1} \approx A\deltax_k + B\deltau_k \label{eq:Ax+Bu}
\end{align}

\todo{gerry}{clean up these objective functions???}
We can also redefine our objective function terms:
\begin{align}
    \norm{x_k-\xd_k}^2 &= \norm{\deltax_k - (\xd_k - \xff_k)}^2 \\
    \norm{u_k-\um}^2 &= \norm{\deltau_k - (\um-\uff_k)}
\end{align}


==> __latexindent_temp.tex <==
We now seek a Kalman Filter to estimate $\xhat_k = E[\deltax_k]$.

==> pgflibraryqrr.shapes.openrectangle.code.tex <==
\let\pgf@sh@openrectangle@full\pgf@sh@bg@rectangle
\let\pgf@sh@openrectangle@\pgf@sh@openrectangle@full
\def\pgf@sh@openrectangle@e    {\pgfsetrectcap\pgfpathmoveto{\SE}\pgfpathlineto{\NE}}
\def\pgf@sh@openrectangle@n    {\pgfsetrectcap\pgfpathmoveto{\NW}\pgfpathlineto{\NE}}
\def\pgf@sh@openrectangle@w    {\pgfsetrectcap\pgfpathmoveto{\SW}\pgfpathlineto{\NW}}
\def\pgf@sh@openrectangle@s    {\pgfsetrectcap\pgfpathmoveto{\SW}\pgfpathlineto{\SE}}
\def\pgf@sh@openrectangle@en{\pgfsetrectcap\pgfpathmoveto{\SE}\pgfpathlineto{\NE}\pgfpathlineto{\NW}}
\def\pgf@sh@openrectangle@ew{\pgfsetrectcap\pgfpathmoveto{\NW}\pgfpathlineto{\SW}\pgfpathmoveto{\SE}\pgfpathlineto{\NE}}
\def\pgf@sh@openrectangle@es{\pgfsetrectcap\pgfpathmoveto{\SW}\pgfpathlineto{\SE}\pgfpathlineto{\NE}}
\def\pgf@sh@openrectangle@enw{\pgfsetbuttcap
  \pgfpathmoveto{\pgfpointadd{\SE}{\pgfpointscale{-1}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}
  \pgfpathlineto{\NE}\pgfpathlineto{\NW}\pgfpathlineto{\pgfpointadd{\SW}{\pgfpointscale{-1}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}}
\def\pgf@sh@openrectangle@ens{\pgfsetbuttcap
  \pgfpathmoveto{\pgfpointadd{\SW}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}
  \pgfpathlineto{\SE}\pgfpathlineto{\NE}\pgfpathlineto{\pgfpointadd{\NW}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}}
\def\pgf@sh@openrectangle@ews{\pgfsetbuttcap
  \pgfpathmoveto{\pgfpointadd{\NE}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}
  \pgfpathlineto{\SE}\pgfpathlineto{\SW}\pgfpathlineto{\pgfpointadd{\NW}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}
\def\pgf@sh@openrectangle@nw{\pgfsetrectcap\pgfpathmoveto{\NE}\pgfpathlineto{\NW}\pgfpathlineto{\SW}}
\def\pgf@sh@openrectangle@ns{\pgfsetrectcap\pgfpathmoveto{\NE}\pgfpathlineto{\NW}\pgfpathmoveto{\SW}\pgfpathlineto{\SE}}
\def\pgf@sh@openrectangle@nws{\pgfsetbuttcap
  \pgfpathmoveto{\pgfpointadd{\NE}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}
  \pgfpathlineto{\NW}\pgfpathlineto{\SW}\pgfpathlineto{\pgfpointadd{\SE}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}
\def\pgf@sh@openrectangle@ws{\pgfsetrectcap\pgfpathmoveto{\NW}\pgfpathlineto{\SW}\pgfpathlineto{\SE}}
\def\pgf@sh@openrectangle@bbg@e{\pgfsetcornersarced{\pgfpointorigin}\pgfpathrectanglecorners{\southwest}{\northeast}}
\let\pgf@sh@openrectangle@bbg@n\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@s\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@w\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@ns\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@ew\pgf@sh@openrectangle@bbg@e
\let\pgf@sh@openrectangle@bbg@full\pgf@sh@openrectangle@full
\let\pgf@sh@openrectangle@bbg@\pgf@sh@openrectangle@
\let\pgf@sh@openrectangle@bbg@enw\pgf@sh@openrectangle@enw
\let\pgf@sh@openrectangle@bbg@ens\pgf@sh@openrectangle@ens
\let\pgf@sh@openrectangle@bbg@ews\pgf@sh@openrectangle@ews
\let\pgf@sh@openrectangle@bbg@nws\pgf@sh@openrectangle@nws
\def\pgf@sh@openrectangle@bbg@en{%
  \pgfpathmoveto{\pgfpointadd{\SE}{\pgfpointscale{-1}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}%
  \pgfpathlineto{\NE}%
  \pgfsetcornersarced{\pgfpointorigin}%
  \pgfpathlineto{\pgfpointadd{\NW}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}%
  \pgfpathlineto{\southwest}}
\def\pgf@sh@openrectangle@bbg@nw{%
  \pgfpathmoveto{\pgfpointadd{\NE}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}%
  \pgfpathlineto{\NW}%
  \pgfsetcornersarced{\pgfpointorigin}%
  \pgfpathlineto{\pgfpointadd{\SW}{\pgfpointscale{-1}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}}%
  \pgfpathlineto{\southwest\pgf@ya\pgf@y\northeast\pgf@y\pgf@ya}}
\def\pgf@sh@openrectangle@bbg@ws{%
  \pgfpathmoveto{\pgfpointadd{\NW}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}%
  \pgfpathlineto{\SW}%
  \pgfsetcornersarced{\pgfpointorigin}%
  \pgfpathlineto{\pgfpointadd{\SE}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}%
  \pgfpathlineto{\northeast}}
\def\pgf@sh@openrectangle@bbg@es{%
  \pgfpathmoveto{\pgfpointadd{\SW}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{+0pt}}}}%
  \pgfpathlineto{\SE}%
  \pgfsetcornersarced{\pgfpointorigin}%
  \pgfpathlineto{\pgfpointadd{\NE}{\pgfpoint{+0pt}{\pgfkeysvalueof{/pgf/outer ysep}}}}%
  \pgfpathlineto{\southwest\pgf@xa\pgf@x\northeast\pgf@x\pgf@xa}}
\pgfset{open rectangle sides/.initial=ns, open rectangle fill/.initial=}
\pgfdeclareshape{open rectangle}{%
  \inheritsavedanchors[from=rectangle]
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}     \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{north west}\inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{north east}\inheritanchor[from=rectangle]{south east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}      \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{base}      \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{base west} \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{base east} \inheritanchor[from=rectangle]{mid east}
  \behindbackgroundpath{%
    \pgfkeysgetvalue{/pgf/open rectangle fill}\pgf@temp
    \ifx\pgf@temp\pgfutil@empty
    \else
      \pgfextract@process\SW{\pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}%
      \pgf@xa\pgf@x\pgf@ya\pgf@y
      \pgfextract@process\NE{\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}}%
      \pgf@xb\pgf@x\pgf@yb\pgf@y
      \pgfextract@process\NW{\pgf@x\pgf@xa\pgf@y\pgf@yb}%
      \pgfextract@process\SE{\pgf@x\pgf@xb\pgf@y\pgf@ya}%
      \csname pgf@sh@openrectangle@bbg@\pgfkeysvalueof{/pgf/open rectangle sides}\endcsname
      \pgfsetfillcolor{\pgfkeysvalueof{/pgf/open rectangle fill}}%
      \pgfusepath{fill}
    \fi
  }%
  \backgroundpath{%
    \pgfextract@process\SW{\pgfpointadd{\southwest}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}%
    \pgf@xa\pgf@x\pgf@ya\pgf@y
    \pgfextract@process\NE{\pgfpointadd{\northeast}{\pgfpointscale{-1}{\pgfpoint{\pgfkeysvalueof{/pgf/outer xsep}}{\pgfkeysvalueof{/pgf/outer ysep}}}}}%
    \pgf@xb\pgf@x\pgf@yb\pgf@y
    \pgfextract@process\NW{\pgf@x\pgf@xa\pgf@y\pgf@yb}%
    \pgfextract@process\SE{\pgf@x\pgf@xb\pgf@y\pgf@ya}%
    \csname pgf@sh@openrectangle@\pgfkeysvalueof{/pgf/open rectangle sides}\endcsname}}
\endinput

